Prism: Semi-Supervised Multi-View Stereo with Monocular Structure Priors

The promise of unsupervised multi-view-stereo (MVS) is to leverage large unlabeled datasets, yet current methods underperform when training on difficult data, such as handheld smartphone videos of indoor scenes. Meanwhile, high-quality synthetic datasets are available but MVS networks trained on these datasets fail to generalize to real-world examples. To bridge this gap, we propose a semi-supervised learning framework that allows us to train on real and rendered images jointly, capturing structural priors from synthetic data while ensuring parity with the real-world domain. Central to our framework is a novel set of losses that leverages powerful existing monocular relative-depth estimators trained on the synthetic dataset, transferring the rich structure of this relative depth to the MVS predictions on unlabeled data. Inspired by perceptual image metrics, we compare the MVS and monocular predictions via a deep feature loss and a multi-scale statistical loss. Our full framework, which we call Prism, achieves large quantitative and qualitative improvements over current unsupervised and synthetic-supervised MVS networks. This is a best-case-scenario result, opening the door to using both unlabeled smartphone videos and photorealistic synthetic datasets for training MVS networks.

==> tbl/addl.tex <==
\begin{table*}[t]
\setlength\tabcolsep{4pt}
% \begin{scriptsize}
\begin{center}
\begin{tabular}{l c c c c|c c c c}
    \thickhline
     & \multicolumn{4}{c|}{ARKit Scenes} & \multicolumn{4}{c}{Hypersim} \\
    \multicolumn{1}{c}{Method} & Abs-rel $\downarrow$ & Abs-diff $\downarrow$ & Abs-inv $\downarrow$ & $\delta < 1.25$ $\uparrow$ & Abs-rel $\downarrow$ & Abs-diff $\downarrow$ & Abs-inv $\downarrow$ & $\delta < 1.25$ $\uparrow$ \\
    \hline
        RC-MVSNet \cite{chang2022rc} & & & & & & & & \\
        CL-MVSNet \cite{xiong2023cl} & & & & & & & & \\
        DIV-MVS \cite{rich2024divloss} & 0.182 & 0.203 & 0.138 & 0.824 & & & & \\
    \hline
        Hypersim Sup & 0.129 & 0.183 & 0.169 & 0.829 & 0.296 & 3.017 & 0.198 & 0.576 \\
        Basic Semi-Sup & 0.127 & 0.165 & 0.108 & 0.873 & \textbf{0.275} & 2.738 & 0.128 & \textbf{0.617} \\
    \hline
        \OURS (ours) & \textbf{0.115} & \textbf{0.148} & \textbf{0.100} & \textbf{0.890} & 0.276 & \textbf{2.654} & \textbf{0.100} & \textbf{0.617} \\
    \hline
\end{tabular}
\end{center}
\vspace{-0.1cm}
\caption{\textbf{Additional Datasets.} This table will contain generalization results on the Hypersim and ARKit Scenes datasets.}
\label{tab:addl}
% \end{scriptsize}
% \vspace{-0.7cm}
\end{table*}

==> tbl/main.tex <==
\begin{table*}[t]
\setlength\tabcolsep{4pt}
% \begin{scriptsize}
\begin{center}
\begin{tabular}{l|c c|c c c c c|g g g}
    \thickhline
    & \multicolumn{2}{c|}{Training Data} & \multicolumn{5}{c|}{Depth Prediction} & \multicolumn{3}{g}{3D Reconstruction} \\
    \multicolumn{1}{c|}{Method} & SN++ & HSim & Abs-rel $\downarrow$ & Abs-diff $\downarrow$ & Abs-inv $\downarrow$ & Sq-rel $\downarrow$ & $\delta < 1.25$ $\uparrow$ & Prec $\uparrow$ & Rec $\uparrow$ & F-score $\uparrow$ \\
    \hline
        RC-MVSNet \cite{chang2022rc} & \greencheck & \redcross & & & & & & & & \\
        CL-MVSNet \cite{xiong2023cl} & \greencheck & \redcross & & & & & & & & \\
        DIV-MVS \cite{rich2024divloss} & \greencheck & \redcross & 0.123 & 0.200 & 0.088 & 0.086 & 0.848 & 0.250 & 0.441 & 0.302 \\
    \hline
        Hypersim Sup & \redcross & \greencheck & 0.118 & 0.215 & 0.133 & 0.086 & 0.831 & & & \\
        Basic Semi-Sup & \greencheck & \greencheck & 0.100 & 0.179 & 0.077 & 0.066 & 0.873 & 0.298 & 0.442 & 0.336 \\
    \hline
        \OURS (ours) & \greencheck & \greencheck & \textbf{0.090} & \textbf{0.158} & \textbf{0.068} & \textbf{0.052} & \textbf{0.895} & \textbf{0.326} & \textbf{0.450} & \textbf{0.359} \\
        \multicolumn{3}{l|}{\hspace{0.75cm}vs. DIV-MVS (unsup SotA)} & {\color{ForestGreen}-26.8\%} & {\color{ForestGreen}-21.1\%} & {\color{ForestGreen}-23.1\%} & {\color{ForestGreen}-39.8\%} & {\color{ForestGreen}+5.6\%} & & & \\
        \multicolumn{3}{l|}{\hspace{0.75cm}vs. Hypersim Sup} & {\color{ForestGreen}-23.7\%} & {\color{ForestGreen}-26.4\%} & {\color{ForestGreen}-49.2\%} & {\color{ForestGreen}-40.0\%} & {\color{ForestGreen}+7.7\%} & & & \\
        \multicolumn{3}{l|}{\hspace{0.75cm}vs. Basic Semi-Sup} & {\color{ForestGreen}-10.0\%} & {\color{ForestGreen}-11.5\%} & {\color{ForestGreen}-11.9\%} & {\color{ForestGreen}-22.2\%} & {\color{ForestGreen}+2.6\%} & & & \\
    \hline
\end{tabular}
\end{center}
\vspace{-0.3cm}
\caption{\textbf{ScanNet++ Dataset.} This table will contain the main evaluation results on the ScanNet++ dataset.}
\label{tab:main}
% \end{scriptsize}
% \vspace{-0.7cm}
\end{table*}
% ---- OLD ----
% \begin{table*}[t]
% \setlength\tabcolsep{7pt}
% % \begin{scriptsize}
% \begin{center}
% \begin{tabular}{l c c c c c|g g g}
%     \thickhline
%     & \multicolumn{5}{c|}{Depth Prediction} & \multicolumn{3}{g}{3D Reconstruction}\\
%     \multicolumn{1}{c}{Method} & Abs-rel $\downarrow$ & Abs-diff $\downarrow$ & Abs-inv $\downarrow$ & Sq-rel $\downarrow$ & $\delta < 1.25$ $\uparrow$ & Prec $\uparrow$ & Rec $\uparrow$ & F-score $\uparrow$ \\
%     \hline
%         Supervised baseline & & & & & & & & \\
%     \hline
%         RC-MVSNet \cite{chang2022rc} & & & & & & & & \\
%         CL-MVSNet \cite{xiong2023cl} & & & & & & & & \\
%         DIV-MVS \cite{rich2024divloss} & 0.121 & 0.190 & 0.088 & 0.080 & 0.858 & 0.362 & 0.392 & 0.368 \\
%         % Hypersim Sup & 0.110 & 0.182 & 0.089 & 0.064 & 0.869 & & & \\
%         % Na\"{i}ve Semi-Sup & 0.101 & 0.169 & 0.076 & 0.062 & 0.884 & & & \\
%         \OURS (ours) & \textbf{0.089} & \textbf{0.150} & \textbf{0.067} & \textbf{0.049} & \textbf{0.905} & \textbf{0.465} & \textbf{0.430} & \textbf{0.439} \\
%     \hline
% \end{tabular}
% \end{center}
% \vspace{-0.1cm}
% \caption{\textbf{ScanNet++ Dataset.} This table will contain the main evaluation results on the ScanNet++ dataset.}
% \label{tab:main}
% % \end{scriptsize}
% % \vspace{-0.7cm}
% \end{table*}

==> tbl/sup.tex <==
\begin{table}[t]
\setlength\tabcolsep{3pt}
% \begin{scriptsize}
\begin{center}
\begin{tabular}{c c c c c}
    \thickhline
    % Monodepth & Abs-rel $\downarrow$ & Abs-diff $\downarrow$ & F-score $\uparrow$ & training examples \\
    & & & \\
    \multirow{-2}{*}{\shortstack[c]{fixed depth\\bounds}} & \multirow{-2}{*}{\shortstack[c]{OOB\\masking}} & \multirow{-2}{*}{Abs-rel $\downarrow$} & \multirow{-2}{*}{Abs-diff $\downarrow$} & \multirow{-2}{*}{$\delta < 1.25$ $\uparrow$} \\
    \thickhline
    & & 0.109 & 0.194 & 0.849 \\
    \checkmark & & 0.102 & 0.171 & 0.879 \\
    \checkmark & \checkmark & \textbf{0.097} & \textbf{0.171} & \textbf{0.881} \\
    \hline
\end{tabular}
\end{center}
\vspace{-0.1cm}
\caption{\textbf{ScanNet++ Dataset.} This table will study how small choices in Hypersim supervision affect cross-dataset transfer.}
\label{tab:sup}
% \end{scriptsize}
% \vspace{-0.7cm}
\end{table}
